Statistical Framework for Clustering MU-MIMO Wireless via Second Order Statistics

This work explores the clustering of wireless users by examining the distances between their channel covariance matrices, which reside on the Riemannian manifold of positive definite matrices. Specifically, we consider an estimator of the Log-Euclidean distance between multiple sample covariance matrices (SCMs) consistent when the number of samples and the observation size grow unbounded at the same rate. Within the context of multi-user MIMO (MU-MIMO) wireless communication systems, we develop a statistical framework that allows to accurate predictions of the clustering algorithm's performance under realistic conditions. Specifically, we present a central limit theorem that establishes the asymptotic Gaussianity of the consistent estimator of the log-Euclidean distance computed over two sample covariance matrices.

==> fig/fig2_grow/fig2_grow_sistem_scn1.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.12157,0.46667,0.70588}%
\definecolor{mycolor2}{rgb}{1.00000,0.00000,1.00000}%
\definecolor{mycolor3}{rgb}{1.00000,0.49804,0.05490}%
\definecolor{mycolor4}{rgb}{0.17255,0.62745,0.17255}%
%
\begin{tikzpicture}

\begin{axis}[%
width=0.75\linewidth,
height=1.0in,
at={(0in,2.1in)},
scale only axis,
scale only axis,
align =center,
xmin=5,
xmax=30,
xlabel style={font=\color{white!15!black}},
xlabel={Growing M},
ymin=0,
ymax=1,
ylabel style={font=\color{white!15!black}},
ylabel={Prob. Clust},
axis background/.style={fill=white},
title style={font=\bfseries},
title={$\text{G = 3, K = 6, }\Delta\text{ d}_\text{g}\text{ = 10}$},
axis x line*=bottom,
axis y line*=left,
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1, line width=2.0pt]
  table[row sep=crcr]{%
5	0.353\\
6	0.387\\
7	0.4396\\
8	0.4916\\
9	0.542\\
10	0.6028\\
11	0.6544\\
12	0.7078\\
13	0.7592\\
14	0.8092\\
15	0.8508\\
16	0.888\\
17	0.9156\\
18	0.9378\\
19	0.9542\\
20	0.9696\\
21	0.9832\\
25	0.993666666666667\\
29	1\\
};
%\addlegendentry{$\text{trad c}_\text{1}\text{ = 2.00, c}_\text{2}\text{ = 2.00, c}_\text{3}\text{ = 2.00}$}

\addplot [color=mycolor1, dashed, line width=2.0pt]
  table[row sep=crcr]{%
5	0.345\\
6	0.390333333333333\\
7	0.465\\
8	0.5386\\
9	0.6216\\
10	0.704\\
11	0.7812\\
12	0.8462\\
13	0.8982\\
14	0.9352\\
15	0.9624\\
16	0.9786\\
17	0.9878\\
18	0.9932\\
19	0.996\\
20	0.9984\\
21	0.9998\\
25	1\\
29	1\\
};
%\addlegendentry{$\text{imp c}_\text{1}\text{ = 2.00, c}_\text{2}\text{ = 2.00, c}_\text{3}\text{ = 2.00}$}

\addplot [color=mycolor2, line width=2.0pt]
  table[row sep=crcr]{%
5	0.254\\
6	0.302\\
7	0.3222\\
8	0.3362\\
9	0.3604\\
10	0.3694\\
11	0.3754\\
12	0.383\\
13	0.4088\\
14	0.412\\
15	0.4272\\
16	0.4388\\
17	0.4684\\
18	0.4826\\
19	0.4996\\
20	0.52\\
21	0.557\\
22	0.581\\
23	0.6138\\
24	0.6426\\
25	0.685\\
26	0.7124\\
27	0.741666666666667\\
29	0.772\\
};
%\addlegendentry{$\text{trad c}_\text{1}\text{ = 1.25, c}_\text{2}\text{ = 1.25, c}_\text{3}\text{ = 1.25}$}

\addplot [color=mycolor2, dashed, line width=2.0pt]
  table[row sep=crcr]{%
5	0.247\\
6	0.315666666666667\\
7	0.3776\\
8	0.4424\\
9	0.5076\\
10	0.5744\\
11	0.634\\
12	0.6966\\
13	0.752\\
14	0.8008\\
15	0.8418\\
16	0.875\\
17	0.907\\
18	0.9336\\
19	0.9544\\
20	0.9708\\
21	0.9858\\
22	0.9944\\
23	0.9982\\
24	0.998\\
25	0.999\\
26	0.9996\\
27	0.999666666666667\\
29	1\\
};
%\addlegendentry{$\text{imp c}_\text{1}\text{ = 1.25, c}_\text{2}\text{ = 1.25, c}_\text{3}\text{ = 1.25}$}

\addplot [color=mycolor3, line width=2.0pt]
  table[row sep=crcr]{%
5	0.201\\
6	0.202666666666667\\
7	0.1664\\
8	0.1362\\
9	0.1228\\
10	0.0838\\
11	0.0656\\
12	0.0516\\
13	0.0496\\
14	0.0388\\
15	0.031\\
16	0.0268\\
17	0.0276\\
18	0.0228\\
19	0.0188\\
20	0.0176\\
21	0.0178\\
22	0.0142\\
23	0.0132\\
24	0.0108\\
25	0.00866666666666667\\
29	0.007\\
};
%\addlegendentry{$\text{trad c}_\text{1}\text{ = 2.00, c}_\text{2}\text{ = 1.50, c}_\text{3}\text{ = 1.25}$}

\addplot [color=mycolor3, dashed, line width=2.0pt]
  table[row sep=crcr]{%
5	0.27\\
6	0.356666666666667\\
7	0.4288\\
8	0.5012\\
9	0.5698\\
10	0.638\\
11	0.7004\\
12	0.7634\\
13	0.8228\\
14	0.8742\\
15	0.9078\\
16	0.9368\\
17	0.961\\
18	0.9738\\
19	0.9836\\
20	0.9916\\
21	0.9966\\
22	0.9978\\
23	0.9992\\
24	0.9992\\
25	0.999666666666667\\
29	1\\
};
%\addlegendentry{$\text{imp c}_\text{1}\text{ = 2.00, c}_\text{2}\text{ = 1.50, c}_\text{3}\text{ = 1.25}$}

\addplot [color=mycolor4, line width=2.0pt]
  table[row sep=crcr]{%
5	0.343\\
6	0.336\\
7	0.333\\
8	0.3324\\
9	0.323\\
10	0.3308\\
11	0.3134\\
12	0.316\\
13	0.3054\\
14	0.317\\
15	0.3044\\
16	0.3348\\
17	0.3418\\
18	0.3688\\
19	0.3764\\
20	0.4194\\
21	0.4662\\
25	0.517\\
29	0.646\\
};
%\addlegendentry{$\text{trad c}_\text{1}\text{ = 2.00, c}_\text{2}\text{ = 1.50, c}_\text{3}\text{ = 1.50}$}

\addplot [color=mycolor4, dashed, line width=2.0pt]
  table[row sep=crcr]{%
5	0.298\\
6	0.359\\
7	0.4334\\
8	0.5068\\
9	0.5812\\
10	0.6672\\
11	0.7392\\
12	0.8014\\
13	0.8578\\
14	0.9048\\
15	0.9324\\
16	0.9604\\
17	0.9782\\
18	0.9888\\
19	0.993\\
20	0.998\\
21	0.9992\\
25	1\\
29	1\\
};
%\addlegendentry{$\text{imp c}_\text{1}\text{ = 2.00, c}_\text{2}\text{ = 1.50, c}_\text{3}\text{ = 1.50}$}

\end{axis}
\end{tikzpicture}%

==> fig/fig2_grow/fig2_grow_sistem_scn2.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.12157,0.46667,0.70588}%
\definecolor{mycolor2}{rgb}{1.00000,0.00000,1.00000}%
\definecolor{mycolor3}{rgb}{1.00000,0.49804,0.05490}%
\definecolor{mycolor4}{rgb}{0.17255,0.62745,0.17255}%
%
\begin{tikzpicture}

\begin{axis}[%
width=0.75\linewidth,
height=1.0in,
at={(0in,2.1in)},
scale only axis,
scale only axis,
align =center,
xmin=5,
xmax=30,
xlabel style={font=\color{white!15!black}},
xlabel={Growing M},
ymin=0,
ymax=1,
ylabel style={font=\color{white!15!black}},
ylabel={Prob. Clust},
axis background/.style={fill=white},
title style={font=\bfseries},
title={$\text{G = 3, K = 15, }\Delta\text{ d}_\text{g}\text{ = 20}$},
axis x line*=bottom,
axis y line*=left,
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1, line width=2.0pt]
  table[row sep=crcr]{%
5	0\\
6	0.00766666666666667\\
7	0.0442\\
8	0.0998\\
9	0.1866\\
10	0.3032\\
11	0.4376\\
12	0.5812\\
13	0.7108\\
14	0.8166\\
15	0.8928\\
16	0.9458\\
17	0.9752\\
21	0.99\\
25	1\\
29	1\\
};
%\addlegendentry{$\text{trad c}_\text{1}\text{ = 2.00, c}_\text{2}\text{ = 2.00, c}_\text{3}\text{ = 2.00}$}

\addplot [color=mycolor1, dashed, line width=2.0pt]
  table[row sep=crcr]{%
5	0\\
6	0.00933333333333333\\
7	0.0696\\
8	0.1514\\
9	0.2758\\
10	0.4348\\
11	0.5946\\
12	0.7442\\
13	0.8596\\
14	0.934\\
15	0.9702\\
16	0.9906\\
17	0.9968\\
21	0.9996\\
25	1\\
29	1\\
};
%\addlegendentry{$\text{imp c}_\text{1}\text{ = 2.00, c}_\text{2}\text{ = 2.00, c}_\text{3}\text{ = 2.00}$}

\addplot [color=mycolor2, line width=2.0pt]
  table[row sep=crcr]{%
5	0\\
6	0.00233333333333333\\
7	0.0122\\
8	0.0234\\
9	0.0518\\
10	0.0904\\
11	0.135\\
12	0.1976\\
13	0.284\\
14	0.3692\\
15	0.449\\
16	0.533\\
17	0.624\\
18	0.6982\\
19	0.7602\\
20	0.8188\\
21	0.8836\\
22	0.9216\\
25	0.957\\
29	0.997\\
};
%\addlegendentry{$\text{trad c}_\text{1}\text{ = 1.25, c}_\text{2}\text{ = 1.25, c}_\text{3}\text{ = 1.25}$}

\addplot [color=mycolor2, dashed, line width=2.0pt]
  table[row sep=crcr]{%
5	0\\
6	0.00533333333333333\\
7	0.0282\\
8	0.0602\\
9	0.1348\\
10	0.2368\\
11	0.3552\\
12	0.4888\\
13	0.6352\\
14	0.7462\\
15	0.833\\
16	0.9032\\
17	0.9516\\
18	0.9726\\
19	0.987\\
20	0.995\\
21	0.9992\\
22	0.9994\\
25	1\\
29	1\\
};
%\addlegendentry{$\text{imp c}_\text{1}\text{ = 1.25, c}_\text{2}\text{ = 1.25, c}_\text{3}\text{ = 1.25}$}

\addplot [color=mycolor3, line width=2.0pt]
  table[row sep=crcr]{%
5	0\\
6	0.000666666666666667\\
7	0.0008\\
8	0.0014\\
9	0.004\\
10	0.005\\
11	0.0056\\
12	0.0074\\
13	0.0154\\
14	0.0192\\
15	0.0248\\
16	0.0328\\
17	0.0536\\
18	0.0698\\
19	0.0864\\
20	0.145\\
21	0.252\\
25	0.340666666666667\\
29	0.579\\
};
%\addlegendentry{$\text{trad c}_\text{1}\text{ = 2.00, c}_\text{2}\text{ = 1.50, c}_\text{3}\text{ = 1.25}$}

\addplot [color=mycolor3, dashed, line width=2.0pt]
  table[row sep=crcr]{%
5	0\\
6	0.006\\
7	0.0496\\
8	0.1096\\
9	0.2132\\
10	0.3482\\
11	0.4938\\
12	0.6352\\
13	0.766\\
14	0.8548\\
15	0.9148\\
16	0.9564\\
17	0.9798\\
18	0.989\\
19	0.9962\\
20	0.998\\
21	0.9992\\
25	1\\
29	1\\
};
%\addlegendentry{$\text{imp c}_\text{1}\text{ = 2.00, c}_\text{2}\text{ = 1.50, c}_\text{3}\text{ = 1.25}$}

\addplot [color=mycolor4, line width=2.0pt]
  table[row sep=crcr]{%
5	0\\
6	0.001\\
7	0.0054\\
8	0.0138\\
9	0.0228\\
10	0.0498\\
11	0.0726\\
12	0.119\\
13	0.1644\\
14	0.2412\\
15	0.3074\\
16	0.4092\\
17	0.5188\\
18	0.6578\\
21	0.771\\
25	0.918666666666667\\
29	0.996\\
};
%\addlegendentry{$\text{trad c}_\text{1}\text{ = 2.00, c}_\text{2}\text{ = 1.50, c}_\text{3}\text{ = 1.50}$}

\addplot [color=mycolor4, dashed, line width=2.0pt]
  table[row sep=crcr]{%
5	0\\
6	0.00966666666666667\\
7	0.0586\\
8	0.127\\
9	0.237\\
10	0.3786\\
11	0.5336\\
12	0.6832\\
13	0.8082\\
14	0.8944\\
15	0.9472\\
16	0.978\\
17	0.9898\\
18	0.9964\\
21	0.9994\\
25	1\\
29	1\\
};
%\addlegendentry{$\text{imp c}_\text{1}\text{ = 2.00, c}_\text{2}\text{ = 1.50, c}_\text{3}\text{ = 1.50}$}

\end{axis}

\begin{axis}[%
width=5.928in,
height=4.299in,
at={(0in,0in)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax=1,
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left
]
\end{axis}
\end{tikzpicture}%

==> fig/fig4_fixedM/fig4_m8_2.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.12157,0.46667,0.70588}%
\definecolor{mycolor2}{rgb}{1.00000,0.00000,1.00000}%
%
\begin{tikzpicture}

\begin{axis}[%
width=0.75\linewidth,
height=1.0in,
at={(0in,2.1in)},
scale only axis,
scale only axis,
align =center,
xmin=5,
xmax=40,
xlabel style={font=\color{white!15!black}},
xlabel={Growing N for fixed M},
ymin=0,
ymax=1,
ylabel style={font=\color{white!15!black}},
ylabel={Prob. Clust},
axis background/.style={fill=white},
title style={font=\bfseries},
title={G = 3, K = 15, M = 8, multipler=1.25 1.25 1.25},
axis x line*=bottom,
axis y line*=left,
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1, line width=2.0pt]
  table[row sep=crcr]{%
9	0.41\\
11	0.59\\
12	0.637\\
13	0.675\\
15	0.744\\
16	0.784\\
16	0.784\\
24	0.878\\
32	0.941\\
40	0.965\\
};
%%\addlegendentry{trad M = 8, K = 9}

\addplot [color=mycolor1, line width=2.0pt, mark=asterisk, mark options={solid, mycolor1}]
  table[row sep=crcr]{%
9	0.512\\
11	0.662\\
12	0.693\\
13	0.735\\
15	0.77\\
16	0.815\\
16	0.815\\
24	0.886\\
32	0.941\\
40	0.965\\
};
%%\addlegendentry{imp M = 8, K = 9}

\addplot [color=mycolor1, dashed, line width=2.0pt]
  table[row sep=crcr]{%
9	0.509837504377216\\
11	0.61653712582984\\
12	0.669340847073593\\
13	0.695167900396177\\
15	0.747269046987292\\
16	0.781763911633989\\
16	0.781763911633989\\
24	0.893739432680243\\
32	0.936861200909644\\
40	0.962745125474032\\
};
%%\addlegendentry{asym M = 8, K = 9}

\addplot [color=mycolor2, line width=2.0pt]
  table[row sep=crcr]{%
9	0.066\\
11	0.116\\
12	0.137\\
13	0.144\\
15	0.191\\
16	0.21\\
16	0.21\\
24	0.305\\
32	0.346\\
40	0.408\\
};
%%\addlegendentry{trad M = 8, K = 15}

\addplot [color=mycolor2, line width=2.0pt, mark=asterisk, mark options={solid, mycolor2}]
  table[row sep=crcr]{%
9	0.146\\
11	0.194\\
12	0.218\\
13	0.211\\
15	0.289\\
16	0.299\\
16	0.299\\
24	0.375\\
32	0.415\\
40	0.477\\
};
%%\addlegendentry{imp M = 8, K = 15}

\addplot [color=mycolor2, dashed, line width=2.0pt]
  table[row sep=crcr]{%
9	0.119414166974076\\
11	0.197721057986213\\
12	0.209926736321171\\
13	0.215410765870303\\
15	0.274155879299471\\
16	0.281623238705126\\
16	0.281623238705126\\
24	0.366449063892705\\
32	0.455023049484862\\
40	0.52749900942441\\
};
%%\addlegendentry{asym M = 8, K = 15}

\end{axis}

\end{tikzpicture}%
